On GPU Implementation for Multi-Precision Integer Division

This paper presents the issues arising in implementing a fast integer division algorithm on general purpose GPUs. The algorithm uses a Newton iteration based on the shifted inverse operation, keeping all arithmetic in the integer domain and relying on data-parallel operators. The principal contribution is an efficient GPU/CUDA implementation for integer precisions from $2^{15}$ to $2^{18}$ -- sizes not supported by \cgbn{} division. We propose algorithmic refinements, define a cost model in terms of multiplications, build on prefix sums and previous work on multi-precision multiplication, and present an evaluation showing near-optimal performance relative to the model for the target precision.

==> table-r16+32.tex <==
\begin{table}[t]
\centering
\begin{minipage}{.3\textwidth}
\begin{tabular}{c@{~~}r@{~~}r}
$m$ & $r_{16}(m)$ & $\dnstrut{2.5ex}\dfrac{2^{16-m}}{15\ln 2}$ \\ \hline
\upstrut{2.5ex}%
1  & 3030 & 3151.64 \\
2  & 1511 & 1575.82 \\
3  & 752  & 787.91 \\
4  & 384  & 393.96 \\
5  & 189  & 196.98 \\
6  & 97   & 98.49 \\
7  & 45   & 49.25 \\
8  & 22   & 24.62 \\
9  & 11   & 12.31 \\
10 & 8    & 6.15 \\
11 & 3    & 3.08 \\
12 & 2    & 1.54 \\
13 & 1    & 0.77 \\
14 & 0    & 0.38 \\
15 & 0    & 0.19 \\
\\
\end{tabular}
\end{minipage}\hfill
\begin{minipage}{.3\textwidth}
\begin{tabular}{c@{~~}r@{~~}r}
$m$ & $r_{32}(m)$ & $\dnstrut{2.5ex}\dfrac{2^{32-m}}{31\ln 2}$ \\
\hline
\upstrut{2.5ex}%
 1 & 98,182,656 & 99,940,774.50 \\
 2 & 49,090,415 & 49,970,387.25 \\
 3 & 24,545,135 & 24,985,193.62 \\
 4 & 12,273,201 & 12,492,596.81 \\
 5 &  6,136,376 &  6,246,298.41 \\
 6 &  3,068,306 &  3,123,149.20 \\
 7 &  1,534,382 &  1,561,574.60 \\
 8 &    766,507 &    780,787.30 \\
 9 &    382,950 &    390,393.65 \\
10 &    191,549 &    195,196.83 \\
11 &     95,658 &     97,598.41 \\
12 &     47,700 &     48,799.21 \\
13 &     23,893 &     24,399.60 \\
14 &     12,052 &     12,199.80 \\
15 &      6,046 &      6,099.90 \\
16 &      3,020 &      3,049.95
\end{tabular}
\end{minipage}~~~~\hfill
\begin{minipage}{.3\textwidth}
\begin{tabular}{c@{~~}r@{~~}r}
$m$ & $r_{32}(m)$ & $\dnstrut{2.5ex}\dfrac{2^{32-m}}{31\ln 2}$ \\
\hline
\upstrut{2.5ex}%
17 & 1540 & 1524.98 \\
18 & 762 & 762.49 \\
19 & 394 & 381.24 \\
20 & 199 & 190.62 \\
21 & 102 & 95.31 \\
22 & 56 & 47.66 \\
23 & 25 & 23.83 \\
24 & 14 & 11.91 \\
25 & 8 & 5.96 \\
26 & 6 & 2.98 \\
27 & 4 & 1.49 \\
28 & 2 & 0.74 \\
29 & 1 & 0.37 \\
30 & 1 & 0.19 \\
31 & 0 & 0.09 \\
32 & 0 & 0.05 \\
\end{tabular}
\end{minipage}

\caption{Estimates and exact counts of $r_{w}(m)$
for $w = 16$ and $32$.}
\label{tbl:r16+32}
\end{table}
